Retinal IPA: Iterative KeyPoints Alignment for Multimodal Retinal Imaging

We propose a novel framework for retinal feature point alignment, designed for learning cross-modality features to enhance matching and registration across multi-modality retinal images. Our model draws on the success of previous learning-based feature detection and description methods. To better leverage unlabeled data and constrain the model to reproduce relevant keypoints, we integrate a keypoint-based segmentation task. It is trained in a self-supervised manner by enforcing segmentation consistency between different augmentations of the same image. By incorporating a keypoint augmented self-supervised layer, we achieve robust feature extraction across modalities. Extensive evaluation on two public datasets and one in-house dataset demonstrates significant improvements in performance for modality-agnostic retinal feature alignment. Our code and model weights are publicly available at \url{https://github.com/MedICL-VU/RetinaIPA}.

==> table_quan.tex <==


\definecolor{fireColor}{RGB}{255,69,0} % Fire dataset color
\definecolor{fireBgColor}{RGB}{255,204,203} % Lighter shade for FIRE dataset background
\definecolor{cfFaColor}{RGB}{30,144,255} % CF-FA dataset color
\definecolor{cfFaBgColor}{RGB}{204,229,255} % Lighter shade for CF-FA dataset background
\definecolor{octSloColor}{RGB}{50,205,50} % OCT-SLO dataset color
\definecolor{octSloBgColor}{RGB}{204,255,204} % Lighter shade for OCT-SLO dataset background


\begin{table}[t]
\centering
\caption{Quantitative results of different model performance in all three datasets}
\small
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{Method} & \multicolumn{5}{c|}{\cellcolor{fireBgColor}\textcolor{fireColor}{FIRE}} & \multicolumn{3}{c|}{\cellcolor{cfFaBgColor}\textcolor{cfFaColor}{CF-FA}} & \multicolumn{3}{c|}{\cellcolor{octSloBgColor}\textcolor{octSloColor}{OCT-SLO}} \\ \hline
\textbf{Method} & \cellcolor{fireBgColor}\textbf{mMEE} & \cellcolor{fireBgColor}\textbf{mMAE} & \cellcolor{fireBgColor}\textbf{$\text{AUC}_{E}$} & \cellcolor{fireBgColor}\textbf{$\text{AUC}_{M}$} & \cellcolor{fireBgColor}\textbf{$\text{AUC}_{H}$} & \cellcolor{cfFaBgColor}\textbf{mMEE} & \cellcolor{cfFaBgColor}\textbf{mMAE} & \cellcolor{cfFaBgColor}\textbf{mAUC} & \cellcolor{octSloBgColor}\textbf{mMEE} & \cellcolor{octSloBgColor}\textbf{mMAE} & \cellcolor{octSloBgColor}\textbf{mAUC} \\ \hline\hline
% Your table data here
SIFT & 1.1 & 1.2 & 1.3 & 1.4 & 1.5 & 1.7 & 1.8 & 1.9 & 2 & 2.1 & 2.2 \\ \hline
REMPE & 1.3 & 1.4 & 1.5 & 1.6 & 1.7 & 1.9 & 2 & 1 & 2 & 2 & 2 \\ \hline
SuperPoint & 1.5 & 1.6 & 1.5 & 1.6 & 1.7 & 2 & 2 & 1 & 3 & 3 & 3 \\ \hline
SuperRetina & 1.5 & 1.6 & 1.5 & 1.6 & 1.7 & 2 & 2 & 1 & 3 & 3 & 3 \\ \hline
Ours & 1.7 & 1.8 & 1.5 & 1.6 & 1.7 & 2.1 & 2 & 1 & 4 & 4 & 4 \\ \hline
\end{tabular}
\end{table}

